Faithful Variable Screening for High-Dimensional Convex Regression

We study the problem of variable selection in convex nonparametric regression. Under the assumption that the true regression function is convex and sparse, we develop a screening procedure to select a subset of variables that contains the relevant variables. Our approach is a two-stage quadratic programming method that estimates a sum of one-dimensional convex functions, followed by one-dimensional concave regression fits on the residuals. In contrast to previous methods for sparse additive models, the optimization is finite dimensional and requires no tuning parameters for smoothness. Under appropriate assumptions, we prove that the procedure is faithful in the population setting, yielding no false negatives. We give a finite sample statistical analysis, and introduce algorithms for efficiently carrying out the required quadratic programs. The approach leads to computational and statistical advantages over fitting a full model, and provides an effective, practical approach to variable screening in convex regression.

==> related_work.tex <==
\section{Related Work}

Variable selection in general nonparametric regression or function
estimation is a notoriously difficult problem. \citet{lafferty2008rodeo} develop a greedy procedure for
adjusting bandwidths in a local linear regression estimator,
and show that the procedure achieves the minimax rate
as if the relevant variables were isolated in advance.
But the method only provably scales to dimensions $p$ that 
grow logarithmically in the sample size $n$, so that $p = O(\log n)$.  Note that this
is the opposite of the high dimensional scaling behavior
known to hold for sparsity selection in linear models
using $\ell_1$ penalization, where the sample size $n$
is logarithmic in the dimension $p$. \citet{bertin:08}
develop an optimization-based approach in
the nonparametric setting, applying the lasso
in a local linear model at each test point.  Here again,
however, the method only scales as $p = O(\log n)$,
the low-dimensional regime.
An approximation theory approach to the same
problem is presented in \cite{devore:11}, 
using techniques based on hierarchical hashing schemes,
similar to those used for ``junta'' problems \cite{mossel:04}.
Here it is shown that the sample complexity scales as $n > \log p$ 
if one adaptively selects the points on
which the high-dimensional function is evaluated.

\citet{dalalyan:12} show that the exponential scaling $p=O(\log n)$ is achievable if the underlying function is assumed to be smooth with respect to a Fourier basis. They also give
support for the intrinsic difficulty of variable
selection in nonparametric regression, giving lower bounds 
showing that sparsistency is not possible if $n < \log p$ or if $n <
\exp s$, where $s$ is the number of relevant variables.
Variable selection over kernel classes is studied
by \citet{Kolch:10}.  

Perhaps most closely related to the present work, is the framework
studied by \cite{Raskutti:12} for sparse additive models, where sparse
regression is considered under an additive assumption, with each
component function belonging to an RKHS.  An advantage of working over
an RKHS, in contrast to the other papers mentioned above, is that
nonparametric regression with a sparsity-inducing regularization penalty can be
formulated as a finite dimensional convex cone optimization.
On the other hand, 
smoothing parameters for the component Hilbert spaces
must be chosen, leading to extra tuning parameters
that are difficult to select in practice.  In addition, 
the additive model must be assumed to
be correct for sparsistent variable selection.

An attraction of the convex function estimation framework we consider
in this paper is that the additive model can be used for convenience,
without assuming it to actually hold.  While nonparametric, the
problem is naturally formulated using finite dimensional convex
optimization, but with no additional tuning parameters.  As we show
below, our method scales to high dimensions, with a dependence on the
intrinsic dimension $s$ that scales polynomially, rather than
exponentially as in the general case analyzed in \cite{dalalyan:12}.


\textbf{Notation.} If
$\mathbf{x}$ is a vector, we use $\mathbf{x}_{-k}$ to denote the
vector with the $k$-th coordinate removed. If $\mathbf{v} \in \R^n$, then
$v_{(1)}$ denotes the smallest coordinate of $\mathbf{v}$ in
magnitude, and $v_{(j)}$ denotes the $j$-th smallest; $\mathbf{1}_n \in \R^n$
is the all ones vector. If $X \in \R^p$ and $S \subset
\{1,...,p\}$, then $X_S$ is the subvector of $X$ restricted to
the coordinates in $S$. Given $n$ samples $X^{(1)},...,X^{(n)}$, we use
$\bar{X}$ to denote the empirical average. Given a random variable $X_k$ and a scalar $x_k$, we use $\E[\cdot \given x_k]$ as a shorthand for $\E[ \cdot \given X_k = x_k]$.


%* Laetitia Comminges, Arnak S. Dalalyan 
%Tight conditions for consistency of variable selection 
%In the context of high dimensionality. 
%Ann. Statist, 40(5), 2667-2696, 2012 
%
%Comment: They estimate the coefficient of the regression function with respect to a Fourier basis and then threshold the estimated coefficients. They prove that sparsistency is achievable so long as $n > log p$ and $n > exp(s)$. They assume that the functions are smooth with respect to the Fourier basis. The fourier coefficients however seem difficult to estimate; it appears that the knowledge of the true density is required. They also provide 
%
%
%* Bertin, K. and Lecu´e, G. (2008). Selection of variables 
%and dimension reduction in high-dimensional non-parametric 
%regression. Electron. J. Stat. 2 1224–1241 
%
%Comment: They assume Holder smoothness and use multiple L1 regularized local polynomial smoothing to detect the sparsity pattern. They require that $p < log n$.
%
%
%* "Approximation of Functions of Few Variables in High Dimensions" 
%by DeVore, Petrova and Wojtaszczyk. 
%
%Comment: They show that variable selection under a scaling of
%

